Recognizing quasi-categorical limits and colimits in homotopy coherent nerves

In this paper we prove that various quasi-categories whose objects are $\infty$-categories in a very general sense are complete: admitting limits indexed by all simplicial sets. This result and others of a similar flavor follow from a general theorem in which we characterize the data that is required to define a limit cone in a quasi-category constructed as a homotopy coherent nerve. Since all quasi-categories arise this way up to equivalence, this analysis covers the general case. Namely, we show that quasi-categorical limit cones may be modeled at the point-set level by pseudo homotopy limit cones, whose shape is governed by the weight for pseudo limits over a homotopy coherent diagram but with the defining universal property up to equivalence, rather than isomorphism, of mapping spaces. Our applications follow from the fact that the $(\infty,1)$-categorical core of an $\infty$-cosmos admits weighted homotopy limits for all flexible weights, which includes in particular the weight for pseudo cones.

==> fibration-cosmoi.tex <==
%!TEX root = all.tex
% ******************************************************************
% ** Title:            On the construction of limits and colimits I of II
% **                   Main file
% ** Precis:
% ** Author:           Emily Riehl and Dominic Verity
% ** Commenced:        23/08/2018
% ******************************************************************

\section{OFFCUT Limits and colimits of (co)cartesian fibrations}\label{sec:limits-of-fibrations}

We conclude this paper with an illustrative application studying limits and colimits of diagrams of (co)cartesian fibrations with a fixed base $B$, considered as subcategories of the sliced $\infty$-cosmos $\eK_{/B}$. In \S\ref{sec:limits-colimits-fibrations}, we prove that the subcategories $\coCart(\eK)_{/B}$ and $\Cart(\eK)_{/B}$ are each closed in $\eK_{/B}$ under flexible weighted limits. It follows, then, that these subcategories are themselves $\infty$-cosmoi with the inclusion defining a functor of such. Our argument is sufficiently general to also show that if the quasi-categorically enriched category $\eK_{/B}$ admits flexibly weighted homotopy colimits satisfying a certain hypothesis, then these are also inherited by the subcategories of cocartesian or cartesian fibrations. This colimit result will be applied in \S\ref{sec:cartesian-monadicity} to prove that the functors of large quasi-categories 
\[ \coCart(\qK)_{/B} \inc \qK_{/B} \qquad \mathrm{and} \qquad \Cart(\qK)_{/B}\inc \qK_{/B}\]
underlying these inclusions are each monadic in the quasi-categorical sense.

\subsection{Limits and colimits of (co)cartesian fibrations}\label{sec:limits-colimits-fibrations}

Let $\pbshape$ denote the category indexing a cospan and write $\eK^\pbshape$ for the simplicially enriched category of cospans in an $\infty$-cosmos $\eK$. Thus, objects of $\eK^\pbshape$ are pairs of maps
  \begin{equation}\label{eq:obj-K-pbshape}
    \xymatrix@=1.5em{
      {} & {B}\ar[d]^f \\
      {C}\ar[r]_g & {A}
    }
  \end{equation}
  and 0-arrows are natural transformations
  \begin{equation}\label{eq:obj-K-pbshape-trans}
    \xymatrix@=1.5em{
      {} & {B}\ar[d]_{f}\ar[dr]^{v} & {} \\
      {C}\ar[r]^{g}\ar[dr]_{w} & {A}\ar[dr]|*+<1pt>{\scriptstyle u} & 
      {B'}\ar[d]^{f'} \\
      {} & {C'}\ar[r]_{g'} & {A'}
    }
  \end{equation}


\begin{obs}
  As with any enriched functor category, $\eK^\pbshape$ inherits limits pointwise from $\eK$. In particular, it  has limits weighted by flexible weights, which are then preserved by the simplicial projection functors $\eK^\pbshape\to\eK$  which evaluate at any object of $\pbshape$.
  \end{obs}

In \cite{RiehlVerity:2013cp}, we introduced a subcategory of $\eK^\pbshape$ (considered here in the dual) whose objects are those diagrams~\eqref{eq:obj-K-pbshape} in which $g$ admits an absolute left lifting through $f$ in the homotopy 2-category of $\eK$, in the sense of Definition \ref{defn:absolute-right-lifting} but with direction of the 2-cells reversed. The 0-arrows in this simplicially enriched category are the \emph{left exact transformations} that we now introduce.

\begin{defn}\label{defn:abs-lift-trans-left-exactness}
Transformations of the kind depicted in~\eqref{eq:obj-K-pbshape-trans} between diagrams which admit absolute left liftings give rise to the following diagram
  \begin{equation}\label{eq:induced-mate}
    \vcenter{
      \xymatrix@=1.5em{
        {} \ar@{}[dr]|(.7){\Uparrow\lambda}
        & {B}\ar[d]^{f}\ar[dr]^{v} & {} \\
        {C}\ar[ur]^{\ell}\ar[r]_{g}\ar[dr]_{w} & 
        {A}\ar[dr]|*+<1pt>{\scriptstyle u} & 
        {B'}\ar[d]^{f'} \\
        {} & {C'}\ar[r]_{g'} & {A'}
      }
    } 
    \mkern40mu = \mkern40mu
    \vcenter{
      \xymatrix@=1.5em{
        {} & {B}\ar[dr]^{v} & {} \\
        {C}\ar[ur]^{\ell}\ar[dr]_{w} & 
        {\scriptstyle\Uparrow\tau}\ar@{}[dr]|(.7){\Uparrow\lambda'} & 
        {B'}\ar[d]^{f'} \\
        {} & {C'}\ar[ur]^{\ell'}\ar[r]_{g'} & {A'}
      }
    } 
  \end{equation}
  in which the triangles are absolute left liftings and the 2-cell $\tau$ is induced by the universal property of the triangle on the right. We say that the transformation \eqref{eq:induced-mate} is {\em left exact\/} if and only if the induced 2-cell $\tau$ is an isomorphism. This left exactness condition holds if and only if, in the diagram on the left, the whiskered 2-cell $u\lambda$ displays $v\ell$ as the absolute left lifting of $g'w$ through $f'$.
\end{defn}


\begin{obs}\label{obs:2-cat-rep-abs-lifting} Unpacking the definitions in any 2-category, $\lambda \colon g \To f\ell$ defines an absolute left lifting diagram if and only if the induced functor 
\begin{equation}\label{eq:rep-lifting-comma-iso} \hom(X,\ell) \comma \hom(X,B) \xrightarrow{\cong} \hom(X,g) \comma \hom(X,f) \end{equation} defines an isomorphism of comma categories, natural in $X$. From the 2-categorical universal property of these comma categories, it is now clear that $\lambda \colon g \To f\ell$ defines an absolute left lifting diagram if and only if
\begin{enumerate}[label=(\roman*)]
\item\label{itm:rep-liftings} for each object $X$, the diagram
\begin{equation}\label{eq:rep.lifting.triangle}
    \xymatrix@R=2em@C=3em{ \ar@{}[dr]|(.7){\Uparrow\hom(X,\lambda)} & \hom(X,B) \ar[d]^{\hom(X,f)} \\ \hom(X,C) \ar[r]_{\hom(X,g)} \ar[ur]^{\hom(X,\ell)} & \hom(X,A)}
    \end{equation}
    defines an absolute left lifting diagram in $\eop{Cat}$, and 
    \item moreoever, each morphism $e \colon Y \to X$ induces a left exact transformation 
    \[    \xymatrix@C=3em@R=2em{
      {} & {\hom(X,B)}\ar[d]_{\hom(X,f)}\ar[dr]^{\hom(e,X)} & {} \\
      {\hom(X,C)}\ar[r]^{\hom(X,g)}\ar[dr]_{\hom(e,X)} & {\hom(X,A)}\ar[dr]|*+<1pt>{\scriptstyle \hom(e,X)} & 
      {\hom(Y,B)}\ar[d]^{\hom(Y,f)} \\
      {} & {\hom(Y,C)}\ar[r]_{\hom(Y,g)} & {\hom(X,A)}
    }
\] 
    \end{enumerate}
    In fact, by the Yoneda lemma, it suffices to assume in \ref{itm:rep-liftings} that $\hom(X,g)$ admits any absolute left lifting along $\hom(X,f)$ for which the transformation induced from any $e \colon Y \to X$ is left exact. Specializing to the case $X=C$ reveals that this absolute left liftings are represented by a morphism $\ell \colon C \to B$ and 2-cell $\lambda \colon g \To f\ell$.
\end{obs}

\begin{defn}
  Let $\eK_{\ell}^\pbshape$ denote the simplicial subcategory of $\eK^\pbshape$ with:
  \begin{itemize}
    \item {\bf objects} those diagrams~\eqref{eq:obj-K-pbshape} in which $g$ admits an absolute left lifting through $f$, and
    \item {\bf $n$-arrows} those $n$-arrows of $\eK^\pbshape$ whose vertices are left exact transformations.
  \end{itemize}
\end{defn}


\begin{lem}\label{lem:absolute-lifting-repleteness}
The inclusion $\eK^\pbshape_\ell \inc \eK^\pbshape$ is replete up to equivalence. That is, given any natural transformation \eqref{eq:obj-K-pbshape-trans} between cospans in $\eK$ that is a pointwise equivalence, then if either cospan admits an absolute left lifting, the other also admits an absolute left lifting defined in such a way that the transformation is left exact. Furthermore, any natural transformation that it pointwise equivalent to a left exact transformation is itself left exact.
\end{lem}
\begin{proof}
A pointwise equivalence \eqref{eq:obj-K-pbshape-trans} induces an isomorphism between the hom-categories appearing in the 2-categorical representable characterization \eqref{eq:rep-lifting-comma-iso} of absolute left lifting diagrams: here if $g$ admits an absolute lifting $\ell \colon C \to B$ through $f$, then the absolute left lifting of $g'$ through $f'$ is defined to be the composite of $\ell$ with $v$ and the equivalence inverse to $w$. As the isomorphism of comma categories for $g'$ and $f'$ is defined by transporting the isomorphism for $g$ and $f$ along $u$, $v$, and $w$, this construction makes the transformation  \eqref{eq:obj-K-pbshape-trans}  exact. The argument for repleteness of 0-arrows is similar.
\end{proof}

In \cite{RiehlVerity:2013cp}, we defined these simplicial categories in order to prove the following proposition, which provided the main ingredient in the proof of Theorem \refIII{thm:limits-in-limits}, mentioned in the proof of Lemma \ref{lem:pullback-colimits}. 


\begin{prop}[{\refIII{prop:abslifts-in-limits}}]
The simplicial subcategory $\qCat^\pbshape_{\ell} \inc \qCat^{\pbshape}$ is closed under flexible weighted limits.
\end{prop}



The proof of Proposition \refIII{prop:abslifts-in-limits} made use of Theorem \refI{thm:pointwise}, which provides a special pointwise characterization of absolute left lifting diagrams between quasi-categories, but nevertheless this result generalizes from $\qCat$ to any $\infty$-cosmos. The proof uses the Yoneda lemma to demonstrate that there is a pullback of simplicial categories:
\[ 
\xymatrix{ \eK^\pbshape_\ell \ar@{^(->}[d] \ar@{^(->}[r]^-y \pbexcursion & (\qCat^\pbshape_\ell)^{\eK\op} \ar@{^(->}[d] \\ \eK^\pbshape  \ar@{^(->}[r]^-y & (\qCat^\pbshape)^{\eK\op}}\]
which tells us that absolute left lifting diagrams in $\eK$ can be characterized representably in $\qCat$ in analogy with the 2-categorical representable characterization of Observation \ref{obs:2-cat-rep-abs-lifting}. Here, however, we require only a corollary of Proposition \refIII{prop:abslifts-in-limits} which generalizes more easily to a quasi-categorically enriched category, without any of the additional structures of an $\infty$-cosmos. So rather than presenting the generalization of Proposition \refIII{prop:abslifts-in-limits}, we instead pursue a proof of Proposition \ref{prop:radj-limits}.

\begin{defn} For a quasi-categorically enriched category $\eC$, let $\Radj(\eC) \inc \eC^\cattwo$ denote the simplicial subcategory of the simplicially-enriched category of arrows $\eC^\cattwo$ with:
  \begin{itemize}
    \item {\bf objects} those morphisms that admit a left adjoint in the homotopy 2-category of $\eC$, and
    \item {\bf $n$-arrows} those $n$-arrows of $\eC^\cattwo$ whose vertices are exact squares,
  \end{itemize}
  where a commutative square between two parallel 0-arrows admitting left adjoints is \emph{exact} if and only if its mate is an isomorphism.
  \begin{equation}\label{eq:exact-square}
    \xymatrix{
      E \ar[d]^p \ar[r]^f & F \ar[d]_q  & &
      E \ar[r]^f & F  & \ar@{}[d]|{\displaystyle \defeq} &
      \ar@{}[dr]|(.7){\Uparrow\eta}  &
      E \ar[r]^f \ar[d]^p & F  \ar@{}[dr]|(.3){\Uparrow\epsilon}
      \ar[d]_q \ar@{=}[r] & F \\
      B \ar@{-->}@/^2ex/[u]^\ell_\dashv \ar[r]_g &
      A \ar@{-->}@/_2ex/[u]_k^\vdash & &
      B \ar@/^2ex/[u]^\ell \ar[r]_g & A \ar@/_2ex/[u]_k
      \ar@{}[ul]\ar@{=>}?(0.35);?(0.65)_{\cong}^{\epsilon_{f\ell}\cdot kg\eta} & &
      B \ar@{=}[r] \ar[ur]^\ell & B \ar[r]_g & A \ar[ur]_k & }
  \end{equation}
\end{defn}

\begin{rmk}[on duals]
Substituting the dual $\eC\co$ of Observation \ref{obs:dual-cosmoi} for $\eC$ exchanges right adjoints with left adjoints: $\Radj(\eC\co) \cong \Ladj(\eC)$. In this way, all of the results appearing below will have duals with ``left'' exchanged with ``right.'' 

As the simplicial categories $\eC$ appearing here are merely quasi-categorically enriched, and not necessarily $\infty$-cosmoi, our results will also apply to the dual $\eC\op$ with the same objects but with
\[ \Fun_{\eC\op}(A,B) \defeq \Fun_{\eC}(B,A).\] This dualization will allow us to conclude results about colimits in $\eC$ from the corresponding statements about limits in $\eC\op$. 
\end{rmk}

\begin{prop}\label{prop:qcat-radj-limits}
The simplicial subcategory admits and the inclusion $\Radj(\qCat) \inc \qCat^\cattwo$ is closed under flexible weighted limits. Moreover, the inclusion $\Radj(\qCat) \inc \qCat^\cattwo$ is replete up to equivalence on objects and 0-arrows.
\end{prop}
\begin{proof}
By Example \ref{ex:radj-lifting}, $p \colon E \to B$ admits a left adjoint if and only if the cospan
\[
\xymatrix{ \ar@{}[dr]|(.7){\Uparrow\eta} & E \ar[d]^p \\ B \ar@{=}[r] \ar@{-->}[ur]^\ell & B}\] admits an absolute left lifting. A square \eqref{eq:exact-square} is exact if and only if the triple $(g,f,g)$ defines a left exact transformation from the cospan $(p,\id_B)$ to the cospan $(q, \id_A)$, the induced 2-cell \eqref{eq:induced-mate} being the desired mate. This proves that we have a pullback diagram of simplicial categories
\[
\xymatrix{ \Radj(\qCat) \ar[r] \ar[d] \pbexcursion & \qCat^\pbshape_\ell \ar@{^(->}[d] \\ \qCat^\cattwo \ar[r]_C & \qCat^\pbshape}\] where the functor $C$ is given by precomposing with the surjective functor $\pbshape \to \cattwo$ that sends one of the arrows to the identity on the codomain object. Proposition \refIII{prop:abslifts-in-limits} proves that the right-hand vertical functor creates flexible weighted limits, and since these are  pointwise defined in $\qCat$, the functor $C$ preserves them. A stricter special case of Lemma \ref{lem:absolute-lifting-repleteness} tells us  that the right-hand vertical functor (and hence also the left-hand vertical functor) is an isofibration. It follows as in the proofs of Lemma \refVI{lem:computad-colimits} and Lemma \ref{lem:pullback-colimits} that $\Radj(\qCat)$ admits and $\Radj(\qCat) \to \qCat^\cattwo$ creates all flexible weighted limits. 

Now this pullback and Lemma \ref{lem:absolute-lifting-repleteness} tells us that the inclusion $\Radj(\qCat)\inc\qCat^\cattwo$ is similarly replete.
\end{proof}

The extension of Proposition \ref{prop:qcat-radj-limits} to any quasi-categorically enriched category $\eC$ makes use of the following representable characterization of adjunctions. 

\begin{prop}\label{prop:representable-adjunctions} Let $\eC$ be a quasi-categorically enriched category. Then \[ 
\xymatrix{ \Radj(\eC) \ar@{^(->}[d] \ar@{^(->}[r]^-y \pbexcursion & \Radj(\qCat)^{\eC\op} \ar@{^(->}[d] \\ \eC^\cattwo  \ar@{^(->}[r]^-y & (\qCat^\cattwo)^{\eC\op}}\] is a pullback diagram of simplicial categories.
  \end{prop}
  
%Here we let $\eC^\cattwo$ and $\qCat^\cattwo$ denote the usual diagram categories, but if $\eC$ is an $\infty$-cosmos the claimed pullback relationship still holds when the objects of $\qCat^\cattwo$ and $\eC^\cattwo$ are isofibrations.
  
\begin{proof} On objects, the pullback asserts that 
\begin{enumerate}[label=(\roman*)]
\item\label{itm:rep-radj} A functor $u \colon A \to B$ admits a left adjoint if and only if for each $X \in \eC$, the functor $\Fun_{\eC}(X,u) \colon \Fun_{\eC}(X,A) \to \Fun_{\eC}(X,B)$ admits a left adjoint and moreover for each $e \colon Y \to X$, the square
\[
  \xymatrix@C=3em{ \Fun_{\eC}(X,A) \ar[d]^-{\Fun_{\eC}(X,u)} \ar[r]^{\Fun_{\eC}(e,A)} & \Fun_{\eC}(Y,A) \ar[d]_{\Fun_{\eC}(Y,u)}  \\ \Fun_{\eC}(X,B) \ar@{-->}@/^2ex/[u]_\dashv^{L_X} \ar[r]_-{\Fun_{\eC}(e,B)} & \Fun_{\eC}(Y,B) \ar@{-->}@/_2ex/[u]^\vdash_{L_Y} }
  \]
  is exact.
  \end{enumerate}
  On 0-arrows, the pullback asserts that moreover:
    \begin{enumerate}[label=(\roman*), resume]
  \item\label{itm:rep-exact} a commutative square between functors admitting left adjoints is exact in $\eC$ if and only if each $\Fun_{\eC}(X,-)$ carries this square to an exact square between quasi-categories.
   \end{enumerate}
The vertical inclusions are full on $n$-arrows for $n>0$, so we need only prove the statements \ref{itm:rep-radj} and \ref{itm:rep-exact}.

The preservation halves of each statement are clear, and the converse direction of \ref{itm:rep-exact} is easy: to test whether a square \eqref{eq:exact-square} is exact, we need to show that a single 2-cell is invertible, and this 2-cell is represented by a 1-arrow in $\Fun_{\eC}(B,F)$. If the square in the image of $\Fun_{\eC}(B,-)$ is exact, then this 1-arrow, as a component of an invertible natural transformation, is an isomorphism, which is what we wanted to show.

For the converse to \ref{itm:rep-radj}, we use the left adjoint $L_B \colon \Fun_{\eC}(B,B) \to \Fun_{\eC}(B,A)$   to define $\ell \colon B \to A$ to be $L_B(\id_B)$. Exactness tells us that for any $b \colon X \to B$, $L_X(b) \cong \ell b \colon X \to A$, from which we infer that the adjointness of $L_X \dashv \Fun_{\eC}(X,u)$ implies that $\Fun_{\eC}(X,\ell) \dashv \Fun_{\eC}(X,u)$ for all $X$, with any $e \colon Y \to X$ defining an \emph{adjunction morphism}, by which we mean a strict exact transformation. Specializing to $X=A$ and $X=B$, we can extract 1-simplices representing the counit and unit of $\ell \dashv u$ as components of the counit and unit at $\id_A$ and $\id_B$. The adjunction morphisms corresponding to precomposition with $u \colon A \to B$ and $\ell \colon B \to A$ are used to verify the triangle identities.
\end{proof}

\begin{comment}


\begin{rmk}\label{rmk:extension-to-htpy} By Lemma \ref{lem:absolute-lifting-repleteness}, Proposition \refIII{prop:abslifts-in-limits} extends to the homotopy limits introduced in Definition \ref{defn:htpy-limit}. Any homotopy limit in $\qCat^{\pbshape}$ is equivalent to the strict flexible weighted limit, which Proposition \refIII{prop:abslifts-in-limits} lifts to $\qCat^\pbshape_{\ell}$. By repleteness of this subcategory, the homotopy limit also lifts.
\end{rmk}



\begin{lem}\label{lem:representable-abs-lifting} Let $\eK$ be an $\infty$-cosmos. 
\begin{enumerate}[label=(\roman*)]
\item\label{itm:rep-abs-lifting} A functor $g \colon C \to A$ admits an absolute left lifting along $f \colon B \to A$ in the homotopy 2-category of $\eK$ if and only if for all $X \in \eK$, the functor $\Fun_{\eK}(X,g)$ admits an absolute left lifting along $\Fun_{\eK}(X,f)$ in the homotopy 2-category of quasi-categories and in addition any $e \colon Y \to X$ induces a left exact transformation
\[    \xymatrix@C=3em@R=2em{
      {} & {\Fun_{\eK}(X,B)}\ar[d]_{\Fun_{\eK}(X,f)}\ar[dr]^{\Fun_{\eK}(e,X)} & {} \\
      {\Fun_{\eK}(X,C)}\ar[r]^{\Fun_{\eK}(X,g)}\ar[dr]_{\Fun_{\eK}(e,X)} & {\Fun_{\eK}(X,A)}\ar[dr]|*+<1pt>{\scriptstyle \Fun_{\eK}(e,X)} & 
      {\Fun_{\eK}(Y,B)}\ar[d]^{\Fun_{\eK}(Y,f)} \\
      {} & {\Fun_{\eK}(Y,C)}\ar[r]_{\Fun_{\eK}(Y,g)} & {\Fun_{\eK}(X,A)}
    }
\] 
Furthermore, a transformation \eqref{eq:obj-K-pbshape-trans} is left exact if and only if the corresponding transformations obtained by applying $\Fun_{\eK}(X,-) \colon \eK \to \qCat$ are left exact for each $X \in \eK$.
\item\label{itm:rep-abs-extension} A functor $f \colon A \to B$  admits an absolute left extension along $g \colon A \to C$  in the homotopy 2-category of $\eK$ if and only if for all $X \in \eK$, the functor $\Fun_{\eK}(g,X)$  admits an absolute left lifting along $\Fun_{\eK}(f,X)$ in $\qCat$ and in addition any $e \colon Y \to X$ induces a left exact transformation. 
\end{enumerate}
\end{lem}
\begin{proof}
We start with \ref{itm:rep-abs-lifting}. Applying Observation \ref{obs:2-cat-rep-abs-lifting} to the homotopy 2-category of quasi-categories, and the universal property of an absolute left lifting $\Fun_{\eK}(X,\ell)$ of  $\Fun_{\eK}(X,g)$ along $\Fun_{\eK}(X,f)$ is encoded by an isomorphism of comma categories
\[ \ho\Fun(Q,\Fun_{\eK}(X,\ell)) \comma \ho\Fun(Q,\Fun_{\eK}(X,B)) \xrightarrow{\cong} \ho\Fun(Q,\Fun_{\eK}(X,g)) \comma \ho\Fun(Q,\Fun_{\eK}(X,f)) \] 
natural in $Q \in \qCat$, where $\ho \colon \qCat \to \eop{Cat}$ is the homotopy category functor. Now simplicial cotensors in an $\infty$-cosmos supply isomorphisms
\[ \Fun_{\qCat}(Q,\Fun_{\eK}(X,B)) \cong \Fun_{\eK}(X, B^Q) \quad \rightsquigarrow\quad \ho\Fun_{\qCat}(Q,\Fun_{\eK}(X,B)) \cong \ho\Fun_{\eK}(X, B^Q).\] Taking $Q=1$, it is now clear from Observation \ref{obs:2-cat-rep-abs-lifting} that the representable absolute lifting property in $\qCat$ implies the absolute left lifting property in $\eK$. To prove the converse, recall that if \eqref{eq:lifting.triangle} defines an absolute lifting triangle in $\eK$ then so does the image of this data under the functor of $\infty$-cosmoi $(-)^Q \colon \eK \to \eK$, a fact which follows easily from the characterization of absolute liftings as equivalences of comma modules given in Proposition \refI{prop:absliftingtranslation}. 

For \ref{itm:rep-abs-extension}, Observation \ref{obs:2-cat-rep-abs-lifting} again tells us that $\Fun_{\eK}(\ell,X) \colon \Fun_{\eK}(C,X) \to \Fun_{\eK}(B,X)$ defines  an absolute left lifting of  $\Fun_{\eK}(g,X) \colon \Fun_{\eK}(C,X) \to \Fun_{\eK}(A,X)$   along $\Fun_{\eK}(f,X)\colon$ $\Fun_{\eK}(B,X) \to \Fun_{\eK}(A,X)$ in the homotopy 2-category of quasi-categories if and only if there is an isomorphism
\[ \ho\Fun(Q,\Fun_{\eK}(\ell,X)) \comma \ho\Fun(Q,\Fun_{\eK}(B,X)) \xrightarrow{\cong} \ho\Fun(Q,\Fun_{\eK}(g,X)) \comma \ho\Fun(Q,\Fun_{\eK}(f,X)) \] 
natural in $Q \in \qCat$. From the cotensor isomorphism
\[  \ho\Fun_{\qCat}(Q,\Fun_{\eK}(B,X))  \cong \ho\Fun_{\eK}(B,X^Q)\] and the dual representable characterization, as in Observation \ref{obs:2-cat-rep-abs-lifting} of absolute left extension diagrams in $\eK$, we see that if $\Fun_{\eK}(g,X)$  admits an absolute left lifting along $\Fun_{\eK}(f,X)$  for which each $e\colon Y \to X$ induces a left exact transformation, then $f$ admits an absolute left extension along $g$, and conversely any absolute left extension supplies an absolute left lifting in $\qCat$ for each $X$ for which each $e \colon Y \to X$ induces a left exact transformation.
\end{proof}
\end{comment}

%We now introduce a class of simplicially enriched limits that generalize both Definition \ref{defn:simp-weight} (by allowing the universal property to be determined up to equivalence, rather than isomorphism) and Definition \ref{defn:htpy-limit} (by considering more general diagram shapes and weights).

%\begin{defn}[flexible weighted homotopy limits]\label{defn:flexible-weighted-htpy} Given a diagram $D \colon \eA \to \eC$ in a quasi-categorically enriched category and a flexible weight $W \colon \eA\op \to \sSet$, a \emph{flexible $W$-weighted homotopy limit} is an object $\{W,D\}^\simeq \in \eC$ equipped with a $W$-shaped cone $W \to \Fun_{\eC}(\{W,D\}^\simeq,D-)$ so that the induced simplicial natural transformation
%\begin{equation}\label{eq:weighted-htpy-UP} \Fun_{\eC}(X,\{W,D\}^\simeq) \we \{W, \Fun_{\eC}(X,D-)\}\end{equation} is an equivalence of quasi-categories for each $X \in \eC$. Here, the right-hand side is the strict $W$-weighted limit of the diagram of quasi-categories $\Fun_{\eC}(X,D-) \colon \eA \to \qCat$. This characterizes the functor represented by $\{W,D\}^\simeq$ as the $W$-weighted homotopy limit of the diagram $\Fun_{\eC}(-,D-) \colon \eA \to \qCat^{\eC\op}$. 
%\end{defn}

%Definition \ref{defn:flexible-weighted-htpy} can be extended to simplicially enriched categories $\eC$ by requiring the map \eqref{eq:weighted-htpy-UP} to be an equivalence of simplicial sets in the Joyal model structure.

\begin{prop}\label{prop:radj-limits}
For any quasi-categorically enriched category $\eC$, $\Radj(\eC)\inc \eC^\cattwo$ is closed under any flexible weighted homotopy limits in $\eC^\cattwo$ that are preserved by the evaluation functors $\dom,\cod \colon \eC^\cattwo \to \eC$. Moreover, if the flexible weighted limit in $\eC^\cattwo$ is strict then so is the flexible weighted limit in $\Radj(\eC)$.
\end{prop}
\begin{proof} 
Consider a diagram
 \[ 
\xymatrix{\eA \ar[r]^-D &  \Radj(\eC) \ar@{^(->}[d] \ar@{^(->}[r]^-y \pbexcursion & \Radj(\qCat)^{\eC\op} \ar@{^(->}[d] \\ & \eC^\cattwo  \ar@{^(->}[r]^-y & (\qCat^\cattwo)^{\eC\op}}\] so that the diagram $D \colon \eA \to \eC^\cattwo$ admits a flexible $W$-weighted homotopy limit $u \colon L \to K$. The hypothesis that this limit is preserved by the domain and codomain functors tells us that the limit cone induces the horizontal natural equivalences
\begin{equation}\label{eq:pointwise-nat-equiv}
\xymatrix{ \Fun_{\eC}(X,L) \ar[r]^-\sim \ar[d]_{\Fun_{\eC}(X,u)} & \{W, \Fun_{\eC}(X,\dom D-) \} \ar[d] \\
  \Fun_{\eC}(X,K) \ar[r]^-\sim & \{W, \Fun_{\eC}(X,\cod D-)\} \ar@{-->}@/_2ex/[u]^\vdash}
  \end{equation}
  
By Proposition \ref{prop:qcat-radj-limits}, the $W$-weighted limit of $yD \colon \eA \to \Radj(\qCat)^{\eC\op}$ exists and is created by the inclusion into $(\qCat^\cattwo)^{\eC\op}$, where it is preserved by the evaluation functors to $\qCat$. Thus, we conclude that $\Fun_{\eC}(-,u) \in (\qCat^\cattwo)^{\eC\op}$ is naturally equivalent to a diagram whose components at each $X \in \eC$, displayed as the right-hand verticals of \eqref{eq:pointwise-nat-equiv}, admit right adjoints and for which the transformations induced by each $e \colon Y \to X$ are exact. The repleteness statement of Proposition \ref{prop:qcat-radj-limits} tells us that an object of $(\qCat^\cattwo)^{\eC\op}$ that is naturally equivalent to an object of $\Radj(\qCat)^{\eC\op}$ is also in $\Radj(\qCat)^{\eC\op}$. Hence,   each component $\Fun_{\eC}(X,u) \colon \Fun_{\eC}(X,L) \to \Fun_{\eC}(X,K)$ admits a right adjoint and the transformations induced by each $e \colon Y \to X$ are exact. Now the pullback of Proposition \ref{prop:representable-adjunctions} tells us that the flexible weighted homotopy limit $u \colon L \to K$ is present in $\Radj(\eC)$. A similar analysis shows that the legs of the limit cone are exact.
\end{proof}

When $\eK$ is an $\infty$-cosmos the previous results restrict to the quasi-categorically enriched categories of arrows or right adjoints in $\eK$ that are isofibrations, for which we re-appropriate the previous notation. If $\eK$ is an $\infty$-cosmos, let $\eK^\cattwo$ denote the $\infty$-\emph{cosmos of isofibrations} of Proposition \ref{prop:isofib-cosmoi}

\begin{prop}\label{prop:radj-cosmos} When $\eK$ is an $\infty$-cosmos, $\Radj(\eK)$ is an $\infty$-cosmos and $\Radj(\eK)\inc\eK^\cattwo$ is a functor of $\infty$-cosmoi, creating isofibrations and simplicially enriched limits.
\end{prop}
\begin{proof}
By Proposition \ref{prop:radj-limits}, isofibrations and strict simplicially enriched limits in $\Radj(\eK)$ are inherited from $\eK^\cattwo$. This proves that the inclusion is a functor of $\infty$-cosmoi. 
\end{proof}



\begin{prop}\label{prop:cocartesian-completeness} Let $\eK$ be an $\infty$-cosmos.
\begin{enumerate}[label=(\roman*)]
\item\label{itm:cocart-limits} The subcategories $\coCart(\eK)_{/B}$ and $\Cart(\eK)_{/B}$ admit and the inclusions \[\coCart(\eK)_{/B} \inc \eK_{/B} \qquad \mathrm{and} \qquad  \Cart(\eK)_{/B} \inc \eK_{/B}\] are closed under homotopy limits with flexible weights.
\item\label{itm:cocart-colimits} The  subcategories $\coCart(\eK)_{/B} \inc \eK_{/B}$ and $\Cart(\eK)_{/B} \inc \eK_{/B}$ are closed under homotopy colimits with flexible weights that are preserved by pullback along $p_0 \colon B^\cattwo \to B$ and $p_1 \colon B^\cattwo \to B$ respectively.
\end{enumerate}
\end{prop}
\begin{proof}
We prove the statements for cocartesian fibrations, the results for cartesian fibrations being dual.   We first argue that there is a pullback of quasi-categorically enriched categories:
\begin{equation}\label{eq:cocart-pullback} \xymatrix{ \coCart(\eK)_{/B} \ar[r] \ar@{^(->}[d] \pbexcursion & \Radj(\eK_{/B}) \ar@{^(->}[d] \\ \eK_{/B} \ar[r]_-K & (\eK_{/B})^\cattwo}\end{equation}
where $K$ is the functor that carries an isofibration $p \colon E \tfib B$ to the isofibration $E^\iso \tfib p \comma B$ over $B$ defined by restricting the Leibniz cotensor $\langle p_0, p \rangle \colon E^\cattwo \tfib p \comma B$ along $E^\iso \tfib E^\cattwo$; recall our convention that the objects in each of these four categories are isofibrations.

We must argue that the claimed pullback relationship holds on objects and 0-arrows. On objects, this  follows from Definition \ref{defn:cocart-fibration}\ref{itm:cocart.fib.chars.ii}, which tells us that $p \colon E \to B$ is cocartesian if and only if the functor $E \to p\comma B$ admits a left adjoint over $B$. This map factors as an equivalence $E \we E^\iso$ followed by the map $E^\iso \tfib p\comma B$, so the composite admits a left adjoint in $\eK_{/B}$ if and only if the map $E^\iso \tfib p \comma B$ does. On 0-arrows, this follows from  Definition \ref{defn:cartesian-functor}, which tells us that a functor 
\[ \xymatrix{ E \ar@{->>}[dr]_p \ar[rr]^f & & F \ar@{->>}[dl]^q \\ & B}\] between cocartesian fibrations is cartesian if and only if the induced outer square
\[    \xymatrix@=1.5em{ {E}\ar[d]_{\rotatebox{90}{$\sim$}}\ar[r]^{f} & {F}\ar[d]^{\rotatebox{90}{$\sim$}} \\ E^\iso \ar[r]^{f^\iso} \ar@{->>}[d] & F^\iso \ar@{->>}[d] \\
   {p\comma B}\ar[r]_{\scriptstyle (f,\id)} & {q\comma B}
    }\]
is exact, and this is the case if and only if the lower square is exact. This tells us that a 0-arrow between cocartesian fibrations in $\eK_{/B}$ defines a cartesian functor if and only if its image under the functor $K$ defines an exact square. Since the pairs of subcategories are full on $n$-arrows for $n >0$, the claimed pullback relationship follows from this pair of results.

Now Proposition \ref{prop:radj-limits} tells us that $\Radj(\eK_{/B})\inc(\eK_{/B})^\cattwo$ creates flexible weighted homotopy limits. The functor  $K\colon \eK_{/B} \to (\eK_{/B})^\cattwo$ preserves them since its construction involves a weighted limit, that commutes with these flexible weighted limits. It follows as in the proof of that result that $\coCart(\eK)_{/B}$ admits flexible weighted limits and both legs of the pullback cone preserve them. In particular the inclusion  $\coCart(\eK)_{/B} \inc \eK_{/B}$ creates flexible weighted limits as claimed, proving \ref{itm:cocart-limits}.

For \ref{itm:cocart-colimits} we apply Proposition \ref{prop:radj-limits} to $\eK\op$, which, while no longer an $\infty$-cosmos, is still quasi-categorically enriched. This tells us that $\Radj(\eK_{/B})\inc (\eK_{/B})^\cattwo$ is closed under flexible weighted homotopy colimits preserved by the domain and codomain evaluation. Now consider a diagram in $\coCart(\eK)_{/B}$ whose flexible weighted homotopy colimit exists in $\eK_{/B}$. The composite $\dom K \colon \eK_{/B} \to \eK_{/B}$ is equivalent to the identity functor, and so preserves all flexible weighted homotopy colimits. For the other composite, note that colimits in $\eK_{/B}$ are created by the projection functor $\Sigma \colon \eK_{/B} \to \eK$, so $\cod K$ preserves colimits if and only if the composite 
\[ \xymatrix{\Sigma \cod K \colon \eK_{/B} \ar[r]^-{p_0^*} & \eK_{/B^\cattwo} \ar[r]^-{\Sigma} & \eK} \] does. In this way, we see that $K$ carries any flexible weighted homotopy colimit preserved by pullback along $p_0 \colon B^\cattwo \to B$ to a flexible weighted homotopy colimit in $(\eK_{/B})^\cattwo$ that is preserved by domain and codomain evaluation. It follows, as above, that  $\coCart(\eK)_{/B}$ admits such colimits formed as in $\eK_{/B}$.
\end{proof}

Proposition \ref{prop:cocartesian-completeness}\ref{itm:cocart-limits} has an interesting and important corollary.

\begin{prop}\label{prop:cartesian-cosmoi} For any $\infty$-category $B$ in an $\infty$-cosmos $\eK$, the quasi-categorically enriched subcategories $\coCart(\eK)_{/B}, \Cart(\eK)_{/B} \subset \eK_{/B}$ spanned by the (co)cartesian fibrations and cartesian functors define $\infty$-cosmoi, with isofibrations and limits inherited from $\eK_{/B}$. The Kan complex enriched subcategories of groupoidal objects are, respectively, the subcategories
\[ \coCart(\eK)\gr_{/B}\inc\coCart(\eK)_{/B} \qquad \mathrm{and} \qquad \Cart(\eK)\gr_{/B}\inc\Cart(\eK)_{/B}\] of groupoidal (co)cartesian fibrations.
\end{prop}
\begin{proof}
Proposition \ref{prop:cocartesian-completeness}\ref{itm:cocart-limits} proves axiom \ref{defn:cosmos}\ref{defn:cosmos:a}. The closure properties of the isofibrations enumerated in axiom \ref{defn:cosmos:b} are inherited from the sliced $\infty$-cosmos. 
\end{proof}

\begin{rmk} The Kan complex enriched category ${}_A\qMod(\eK)_B$ of modules from $A$ to $B$ in an $\infty$-cosmos $\eK$ is also the category of groupoidal objects in an $\infty$-cosmos, namely the $\infty$-cosmos of \emph{two-sided fibrations} that will be introduced in a forthcoming paper \cite{RiehlVerity:2017ts}.
\end{rmk}

%\begin{proof} By Theorem \ref{thm:complete-objects}, to show that a quasi-category is complete, it suffices to show that it has small products, pullbacks, and sequential limits.  Proposition \ref{prop:general-homotopy-limits} explains how each of these may be constructed in quasi-categories arising as homotopy coherent nerves of Kan-complex enriched categories: Proposition \ref{prop:homotopy-products}, Example \ref{ex:ho-pullbacks}, and Example \ref{ex:ho-towers} describe the special cases of products, pullbacks, and sequential limits respectively. 

%For instance, Example \ref{ex:qcat-cosmos} applies these results to prove that the large quasi-category $\qqCat_{/B}$ is complete, with each of these limit constructions modeled at the simplicial category of fibrant objects level by the familiar homotopy limit constructions. It remains only to argue that $\coCart_{/B} \subset \qqCat_{/B}$ is closed under these limit constructions.

%The product of a family of objects $(p_i \colon E_i \tfib B)_{i \in I}$ in $\qqCat_{/B}$ is formed by the pullback\[ \xymatrix{ \prod_{i,B} E_i \ar@{->>}[d]_{\prod_{i \in I} p_i} \ar[r] \pbexcursion & \prod_{i \in I} E_i \ar@{->>}[d]^{\prod_{i \in I} p_i} \\ B \ar[r]_-\Delta & \prod_{i \in I} B}\] If each $p_i$ is a cocartesian fibration, so is $\prod_{i \in I} p_i$ and thus also their pullback, proving that $\coCart_{/B} \subset \qqCat_{/B}$ is closed under products.
%\end{proof}




\subsection{Monadicity of (co)cartesian fibrations}\label{sec:cartesian-monadicity}

We now show that the homotopy coherent nerves of the maximal Kan complex enriched subcategories of
\[ \coCart(\eK)_{/B} \inc \eK_{/B} \qquad \mathrm{and} \qquad \Cart(\eK)_{/B}\inc \eK_{/B}\]
are monadic as functors between large quasi-categories.

\begin{thm}\label{thm:cartesian-monadicity} Let $B$ be an object in an $\infty$-cosmos $\eK$. Then the functors 
\[ \coCart(\qK)_{/B} \inc \qK_{/B} \qquad \mathrm{and} \qquad \Cart(\qK)_{/B}\inc \qK_{/B}\]
are monadic.
\end{thm}

We prove Theorem \ref{thm:cartesian-monadicity} using the $\infty$-categorical monadicity theorem, Theorem \refII{thm:monadicity} from \cite{RiehlVerity:2012hc}.

\begin{thm}[{monadicity; \refII{thm:monadicity}}]\label{thm:monadicity} Let $u \colon A \to B$ be a functor between $\infty$-categories. If 
\begin{enumerate}[label=(\roman*)]
\item\label{itm:monadicity-adj} $u$ admits a left adjoint,
\item\label{itm:monadicity-split} $A$ admits and $u$ preserves colimits of $u$-split simplicial objects, and
\item\label{itm:monadicity-conserv} $u$ is conservative,
\end{enumerate}
then the adjunction is monadic, i.e., $A$ is equivalent to the $\infty$-category of algebras for the homotopy coherent monad on $B$ underlying the corresponding homotopy coherent adjunction.
\end{thm}

For more about homotopy coherent monads and monadicity see \S\refII{sec:formal}-\refII{sec:monadicity}.  One ingredient of our proof will make use of the  quasi-categorical version of Proposition \ref{prop:cocartesian-completeness}.

\begin{cor}\label{cor:qcocartesian-completeness} Let $\eK$ be an $\infty$-cosmos and $B \in \eK$ be any $\infty$-category.
\begin{enumerate}[label=(\roman*)]
\item\label{itm:qcocart-limits} The quasi-category $\coCart(\qK)_{/B}$ is complete  $\coCart(\qK)_{/B} \inc \qK_{/B}$ is closed under limits.
\item\label{itm:qcocart-colimits} The inclusion  $\coCart(\qK)_{/B} \inc \qK_{/B}$ is closed under colimits preserved by pullback along $p_0 \colon B^\cattwo \to B$.
\end{enumerate}
\end{cor}
\begin{proof}
Proposition \ref{prop:cartesian-cosmoi} proves that $\coCart(\eK)_{/B}$ is an $\infty$-cosmos, so Proposition \ref{prop:qcat-cosmos} implies that the quasi-category $\coCart(\qK)_{/B}$ is complete. The proof of that result constructs limits in the quasi-category as flexible $\widetilde{W}$-weighted limits in $g_*\coCart(\eK)_{/B}$, where $\widetilde{W}$ is a replacement of the weight $W$ of Definition \ref{defn:htpy-limit}. The $\widetilde{W}$-weighted limits are inherited from the $\infty$-cosmos $\coCart(\eK)_{/B}$. Since Proposiiton \ref{prop:cocartesian-completeness} demonstrates that flexible weighted limits are created by the inclusion $\coCart(\eK)_{/B}\inc\eK_{/B}$ and the diagram of inclusions is a pullback
\[ \xymatrix{ g_*\coCart(\eK)_{/B} \pbexcursion \ar@{^(->}[r] \ar@{^(->}[d] & g_*\eK_{/B} \ar@{^(->}[d] \\ \coCart(\eK)_{/B} \ar@{^(->}[r] & \eK_{/B}}\]
this tells us that $\coCart(\qK)_{/B} \inc \qK_{/B}$ is closed under limits.

To prove \ref{itm:qcocart-colimits}, the pullback of quasi-categorically enriched categories \eqref{eq:cocart-pullback} passes to a pullback of maximal Kan complex enriched categories, and hence to a pullback of quasi-categories upon applying the homotopy coherent nerves. The dual of Proposition \ref{prop:general-homotopy-limits} tells us colimits in $\coCart(\qK)_{/B}$ are modeled by homotopy colimits in $g_*\coCart(\eK)_{/B}$,
and such homotopy colimits have flexible weights. These is turn are modeled by flexible weighted homotopy colimits in $\coCart(\eK)_{/B}$ with a modified weight. The claimed result now follows from Proposition \ref{prop:cocartesian-completeness}\ref{itm:cocart-colimits} and Lemma \ref{lem:pullback-colimits}.
\end{proof}


We next construct the left adjoints, which make use of the Yoneda lemma for (co)cartesian fibrations, whose statement we now recall in the dual.

\begin{thm}[{Yoneda lemma; \refIV{thm:yoneda}}]\label{thm:yoneda} Consider the cocartesian fibration $p_1 \colon b\comma B \tfib B$ associated to an element $b \colon 1 \to B$ in an $\infty$-category $B$ in an $\infty$-cosmos $\eK$. Then for any cocartesian fibration $p \colon E \tfib B$, restriction along the canonical element $i \colon 1 \to b \comma B$ corresponding to the identity on $b$ induces an equivalence of quasi-categories
\[ \Fun_{\coCart(\eK)_{/B}}( p_1 \colon b\comma B\tfib B, p \colon E \tfib B) \we \Fun_{\eK_{/B}}(b \colon 1 \to B, p \colon E \tfib B).\] 
\end{thm}



\begin{prop}\label{prop:cartesian-reflection} For any $\infty$-category $B$ in an $\infty$-cosmos $\eK$, the forgetful functors admit left adjoints
\[ \adjdisplay L -| U : \coCart(\qK)_{/B} -> \qK_{/B}. \qquad \mathrm{and} \qquad \adjdisplay L -| U : \Cart(\qK)_{/B} -> \qK_{/B}.\]
defined respectively by
\[ \xymatrix@R=1.5em{ \coCart(\qK)_{/B} & \qK_{/B} \ar[l]_-L \ar[r]^-L & \Cart(\qK)_{/B} \\ f \comma B \ar@{->>}[d]_{p_1} & A \ar[d]^f \ar@{}[dl]|\mapsfrom \ar@{}[dr]|{\displaystyle\mapsto} & B \comma f \ar@{->>}[d]^{p_0} \\ B & B & B}\]
\end{prop}
\begin{proof}
We construct the left adjoint to the inclusion of cocartesian fibrations into the slice, the construction for cartesian fibrations being dual. Consider a functor $f \colon A \to B$ and a cocartesian fibration $p \colon E \tfib B$ and write $\pi \colon B \times A \tfib B$ for the projection. The adjunction 
\[\adjdisplay {\pi \circ -} -| \pi^* : \eK_{/B} -> \eK_{/B \times A}.\] provides a natural isomorphism
\[ \Fun_{\eK_{/B}}(f \comma B \xtfib{p_1} B, E \xtfib{p} B) \cong \Fun_{\eK_{/B \times A}}(f \comma B \xtfib{(p_1,p_0)} B \times A, E \times A \xtfib{p \times \id} B \times A).\] The slice $\infty$-cosmos $\eK_{/B \times A}$ is isomorphic to the slice $(\eK_{/A})_{/\pi}$ of the $\infty$-cosmos $\eK_{/A}$ over the object $\pi \colon B \times A \tfib A$. The morphisms
\[ \xymatrix{ f \comma B \ar@{->>}[dr]_{p_0}\ar[rr]^{(p_1,p_0)} & & B \times A \ar@{->>}[dl]^\pi & & E \times A \ar@{->>}[dr] \ar[rr]^{p \times \id}& & B \times A \ar@{->>}[dl]^\pi \\ & A & & & & A}\] each define cocartesian fibrations in $\eK_{/A}$ with the same codomain object $\pi$. In the first instance, this is because the isofibration $(p_1,p_0) \colon f \comma B \tfib B \times A$ is a \emph{cocartesian fibration on the left}; see Corollary \refV{cor:comma-is-a-module}. In the latter case, this follows from the fact that $- \times A \colon \eK \to \eK_{/A}$ defines a functor of $\infty$-cosmoi.

We argue that the adjoint correspondence restricts to define an isomorphism
%\[ \Fun^c_{B}(f \comma B \xtfib{p_1} B, E \xtfib{p} B) \cong \Fun^c_{B \times A}(f \comma B \xtfib{(p_1,p_0)} B \times A, E \times A \xtfib{p \times \id} B \times A)\]
 between those functors over $B$ that are cartesian functors in $\eK_{/B}$ and those functors over $\pi \colon B \times A \tfib A$ that are cartesian functors in $\eK_{/A}$, i.e., provides an isomorphism
\begin{equation}\label{eq:first-iso} \Fun_{\coCart(\eK)_{/B}}(f \comma B \tfib B, E \tfib B) \cong \Fun_{\coCart(\eK_{/A})_{/\pi}}(f \comma B \tfib B \times A, E \times A \tfib B \times A).\end{equation} To see this note that the adjoint transpose of a functor $g \colon f \comma B \to E$ over $B$ is the functor
\[ \xymatrix{ f \comma B \ar@{->>}[dr]_{(p_1,p_0)} \ar[rr]^{(g, p_0)} & & E \times A \ar@{->>}[dl]^{p \times \id} \\ & B \times A}\] 
The $p \times \id$-cocartesian cells in $\eK_{/A}$ are precisely those cells whose component in $E$ is $p$-cartesian. Thus it is clear that if $g$ is a cartesian functor over $B$ then $(g,p_0)$ is a cartesian functor over $B \times A$. For the converse, we appeal to Lemma \refV{lem:two-sided-groupoidal-cells}, which tells us that the $p_1$-cartesian cells are precisely those 2-cells $\chi$ with codomain $f \comma B$ for which $p_0\chi$ is an isomorphism. Each such 2-cell is isomorphic in $\eK$ to a 2-cell for which $p_0\chi$ is an identity, i.e., to a 2-cell in $\eK_{/A}$. Thus if $(g,p_0)$ is a cartesian functor over $A \times B$, then $g$ is a cartesian functor over $B$.

Recall that the terminal object in $\eK_{/A}$ is the identity on $A$. In particular, the object $\pi \colon B \times A \tfib A$ in $\eK_{/A}$ has an element 
\[ \xymatrix{ A \ar[rr]^-{(f,\id)} \ar@{=}[dr] & & B \times A \ar@{->>}[dl]^\pi \\ & A}\]
for which the associated contravariant comma module is $(p_1,p_0) \colon f \comma B \tfib B \times A$. Applying the Yoneda lemma of Theorem \ref{thm:yoneda} in $\eK_{/A}$, we see that restriction along
\[ \xymatrix{ A \ar[dr]_{(f,\id)} \ar[rr]^-i & & f \comma B \ar@{->>}[dl]^{(p_1,p_0)} \\ & B\times A}\] induces an equivalence
\[\Fun_{\coCart(\eK_{/A})_{/\pi}}(f \comma B \tfib B \times A, E \times A \tfib B \times A) \we \Fun_{\eK_{/B \times A}}( A  \xrightarrow{(f,\id)} B \times A,E \times A \tfib B \times A). \] 
Composing with the isomorphisms \eqref{eq:first-iso} and 
\[\Fun_{\eK_{/B \times A}}(A \xrightarrow{(f,\id)} B \times A,E \times A \xtfib{p \times \id} B \times A) \cong \Fun_{\eK_{/B}}(A \xrightarrow{f} B, E \xtfib{p} B)\] completes the proof.
\end{proof}

\begin{lem}\label{lem:cartesian-functor-conservativity} In any commutative diagram
\[ \xymatrix{ E \ar[rr]^f \ar@{->>}[dr]_p & & F \ar@{->>}[dl]^q \\ & B}\]
where $f$ is an equivalence and $p$ and $q$ are both cartesian fibrations or both cocartesian fibrations, then $f$ is a cartesian functor.
\end{lem}
\begin{proof}
Proposition \refI{prop:equivtoadjoint} observes that any equivalence may be promoted to an adjoint equivalence, with the equivalence defining either (or in fact both) the left or right adjoint. Corollary \refIV{cor:radj-cartesian} proves that any right adjoint between cartesian fibrations is a cartesian functor; dually any left adjoint between cocartesian fibrations is a cartesian functor. So the result follows.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:cartesian-monadicity}]
Proposition \ref{prop:cartesian-reflection} verifies hypothesis \ref{itm:monadicity-adj} of Theorem \ref{thm:monadicity} and Lemma \ref{lem:cartesian-functor-conservativity} is stronger than hypothesis  \ref{itm:monadicity-conserv}. It remains only to verify hypothesis \ref{itm:monadicity-split}. In this context, a $u$-split simplicial object is given by a diagram of quasi-categories
\[ \xymatrix{ \Del\op \ar[r] \ar@{^(->}[d] & \coCart(\qK)_{/B} \ar[d]^u \\ \Del[t] \ar[r] & \qK_{/B}}\] The diagram $\Del[t] \to \qK_{/B}$ is a \emph{split simplicial object}, which Theorem \refI{thm:splitgeorealizations} proves is an \emph{absolute} colimit diagram: in any quasi-category $\qQ$, the final object of a diagram $\Del[t] \to \qQ$ is the colimit of the underlying simplicial object $\Del\op\inc\Del[t] \to \qQ$ and such colimits are preserved by any functor. So the hypothesis of Corollary \ref{cor:qcocartesian-completeness}\ref{itm:qcocart-colimits} is satisfied, and we conclude that $\coCart(\qK)_{/B}$ admits such colimits and $\coCart(\qK)_{/B} \to \qK_{/B}$ preserves them. Theorem \ref{thm:monadicity}  now tells us that this functor is monadic, as claimed.
\end{proof}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "all"
%%% End:

